Bag of Negatives for Siamese Architectures

Training a Siamese architecture for re-identification with a large number of identities is a challenging task due to the difficulty of finding relevant negative samples efficiently. In this work we present Bag of Negatives (BoN), a method for accelerated and improved training of Siamese networks that scales well on datasets with a very large number of identities. BoN is an efficient and loss-independent method, able to select a bag of high quality negatives, based on a novel online hashing strategy.

==> bin1.tex <==
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/0.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/1.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/2.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/3.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/4.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/5.jpg}
 
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/6.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/7.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/8.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/9.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/10.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/11.jpg}
  
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/12.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/13.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/14.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/15.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/16.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/6/17.jpg}
  %\caption{Samples from two bins.}
  %\label{fig:two_bins}
%\end{figure}

==> bin3.tex <==
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/0.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/1.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/2.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/3.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/4.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/5.jpg}
  
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/6.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/7.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/8.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/9.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/10.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/11.jpg}
  
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/12.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/13.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/14.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/15.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/16.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/5/17.jpg}

==> bin4.tex <==
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/0.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/1.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/2.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/3.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/4.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/5.jpg}
  
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/6.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/7.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/8.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/9.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/10.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/11.jpg}
  
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/12.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/13.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/14.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/15.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/16.jpg}
\includegraphics[width=0.145\linewidth, height=0.4\linewidth]{figs/subspaces/73/17.jpg}
